Generalizing Homophily to Simplicial Complexes

Group interactions occur frequently in social settings, yet their properties beyond pairwise relationships in network models remain unexplored. In this work, we study homophily, the nearly ubiquitous phenomena wherein similar individuals are more likely than random to form connections with one another, and define it on simplicial complexes, a generalization of network models that goes beyond dyadic interactions. While some group homophily definitions have been proposed in the literature, we provide theoretical and empirical evidence that prior definitions mostly inherit properties of homophily in pairwise interactions rather than capture the homophily of group dynamics. Hence, we propose a new measure, $k$-simplicial homophily, which properly identifies homophily in group dynamics. Across 16 empirical networks, $k$-simplicial homophily provides information uncorrelated with homophily measures on pairwise interactions. Moreover, we show the empirical value of $k$-simplicial homophily in identifying when metadata on nodes is useful for predicting group interactions, whereas previous measures are uninformative.

==> figures/data.tex <==
\begin{table}[htbp]\centering
\caption{Datasets used in our experiments}
\begin{tabular}{l*{3}{c}}
\hline\hline
\multicolumn{1}{c}{Name} &\multicolumn{1}{c}{Nodes}&\multicolumn{1}{c}{Edges}&\multicolumn{1}{c}{Triangles}\\
            
\hline
Enron  &       2.154&       1.669&       1.669\\
[1em]
DBLP   &      (0.33)&      (0.034)&      (0.034)\\
[1em]
contact-high-school  &            &            &     0.00031\\
[1em]
contact-primary-school   &            &            &      (0.00)\\
[1em]
\hline\hline
\multicolumn{4}{p{0.6\linewidth}}{\footnotesize{Notes: }}\\
\end{tabular}
\end{table}


==> figures/homophily-defns-mathematical.tex <==
% Definitions of homophily

==> figures/triad-defns.tex <==
\begin{figure}[ht]
  \centering
  \parbox{\figrasterwd}{
    \parbox{.6\figrasterwd}{%
      \subcaptionbox{}{\includegraphics[width=\hsize, height=8cm]{imageA}}%'height=8cm' is needed for this example only and can be dropped when using it with actual images
    }
    \hskip1em
    \parbox{.3\figrasterwd}{%
      \subcaptionbox{}{\includegraphics[width=\hsize]{imageB}}
      \vskip1em
      \subcaptionbox{}{\includegraphics[width=\hsize]{imageC}}  
    }
  }
\end{figure}

==> tables/prediction-data.tex <==
\begin{table*}[ht]
    \centering
    \caption{Summary statistics for timestamped data used in link prediction. \textcolor{red}{TODO: Merge this table with Table 1}}
    \label{tab:prediction_data}
    \begin{tabular}{lrrrrr}
\toprule
                         Dataset &    nodes & classes &       edges &    triangles & unique timesteps \\
\midrule
       \texttt{cont-hospital} \cite{genois2018can} &       81 &       5 &     150,126 &      194,526 &    12,605 \\
   \texttt{cont-workplace-13} \cite{genois2018can} &      100 &       5 &     394,247 &    1,556,114 &    20,129 \\
   \texttt{cont-workplace-15} \cite{genois2018can} &      232 &      12 &   1,283,194 &   14,400,056 &    21,536 \\
 \texttt{cont-primary-school} \cite{genois2018can} &      242 &      11 &   6,594,492 &  214,546,490 &     3,124 \\
           \texttt{bills-senate} \cite{fowler2006connecting, fowler2006legislative} &      297 &       4 &      35,993 &       27,850 &     4,975 \\
    \texttt{cont-high-school} \cite{genois2018can} &      332 &       9 &  18,613,039 &  432,483,820 &     8,938 \\
            \texttt{bills-house} \cite{fowler2006connecting, fowler2006legislative} &    1,495 &       * &      48,086 &       39,236 &     4,871 \\
                   \texttt{hosp-DAWN} \cite{benson2018simplicial} &    2,558 &     364 &   2,346,571 &    5,092,922 &         8 \\
            \texttt{coauth-dblp} \cite{agarwal2016women} &  105,256 &       2 &     415,492 &      824,240 &        55 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/ssbm-results.tex <==
\begin{table}[t!]
    \centering
    \begin{tabular}{lr} \toprule
\multicolumn{2}{c}{Model Parameters} \\ 
\midrule
Classes                       &                          2 \\
Group Size                     &       1,000\\
($p_1$, $q_1$)           & ($0.05$, $0.01$)  \\
($p_2$, $q_2$)           & ($0.15$, $0.70$)  \\ \midrule
\multicolumn{2}{c}{Observed Counts} \\ \midrule
$\#$ Filled Triangles            &     29,215.86 ($\pm$470.15) \\
$\#$ Homopilous Filled Triangles  &     18,747.99 ($\pm$348.86) \\
$\#$ Closed Triangles             &  140,080.89 ($\pm$1,765.56) \\
$\#$ Homophilous Closed Triangles  &  125,118.30 ($\pm$1,673.39) \\  \midrule
\multicolumn{2}{c}{Scores} \\\midrule
Node Baseline                &           2.57 ($\pm$ 0.029) \\
Edge Baseline &           0.72 ($\pm$ 0.006) \\
\bottomrule
\end{tabular}
    \caption{Summary of results on the simplicial stochastic block model. Actually, will replace this with line plots showing homophily scores as a function of $p_1/q_1$ and $p_2/q_2$.}
    \label{tab:ssbm_results}
\end{table}
